TPCap: Unlocking Zero-Shot Image Captioning with Trigger-Augmented and Multi-Modal Purification Modules

Recent advancements in large language models (LLMs) have significantly enhanced the fluency and logical coherence of image captioning. Retrieval-Augmented Generation (RAG) is widely adopted to incorporate external knowledge into LLMs; however, existing RAG-based methods rely on separate retrieval banks, introducing computational overhead and limiting the utilization of LLMs' inherent zero-shot capabilities. To address these limitations, we propose TPCap, a novel trigger-augmented and multi-modal purification framework for zero-shot image captioning without external retrieval libraries. TPCap consists of two key components: trigger-augmented (TA) generation and multi-modal purification (MP). The TA module employs a trigger projector with frozen and learnable projections to activate LLMs' contextual reasoning, enhance visual-textual alignment, and mitigate data bias. The MP module further refines the generated entity-related information by filtering noise and enhancing feature quality, ensuring more precise and factually consistent captions. We evaluate TPCap on COCO, NoCaps, Flickr30k, and WHOOPS datasets. With only 0.82M trainable parameters and training on a single NVIDIA RTX 4090 GPU, TPCap achieves competitive performance comparable to state-of-the-art models.

==> tab_trigger_projector.tex <==
\begin{table}[tb]
{	\centering
	\caption{
		Ablations of design choices for the proposed trigger projector in each trigger augmented module show that the combination of a learnable linear and a frozen pre-trained linear architecture works the best.
	}\label{fig_5}

		
		\resizebox{\linewidth}{!}{
		\begin{threeparttable}
		\begin{tabular}{l|cc|cc|cc|cc|cc|cc}
			\toprule[1pt]
			\multirow{2}{*}{\textbf{Module}} & 
			\multicolumn{2}{c|}{a} & 
			\multicolumn{2}{c|}{b} & 
			\multicolumn{2}{c|}{c} & 
			\multicolumn{2}{c|}{d} & 
			\multicolumn{2}{c|}{e} & 
			\multicolumn{2}{c}{f} \\
			& \multicolumn{1}{c} {TA1} &
			\multicolumn{1}{c|} {TA2} &
			\multicolumn{1}{c} {TA1} &
			\multicolumn{1}{c|} {TA2} &
			\multicolumn{1}{c} {TA1} &
			\multicolumn{1}{c|} {TA2} &
			\multicolumn{1}{c} {TA1} &
			\multicolumn{1}{c|} {TA2} &
			\multicolumn{1}{c} {TA1} &
			\multicolumn{1}{c|} {TA2} &
			\multicolumn{1}{c} {TA1} &
			\multicolumn{1}{c} {TA2} \\
			\midrule
			Linear & $\times$ & $\times$ & & & & & $\times$ & & & $\times$ & &  \\
			Shared Linear & &  & $\times$ & $\times$ & $\times$ * & $\times$ * & & $\times$ & $\times$ & & $\times$ & $\times$ \\
			Frozen Linear & & & & & & & & * & * & & * & * \\
			\bottomrule
		\end{tabular}
			\begin{tablenotes}
			\footnotesize
			\item The $\times$ and * denote the order in which modules, such as the "f" column, indicates that the features first go through a shared linear layer and then through a frozen linear layer.
		\end{tablenotes}
		\end{threeparttable}
	}

}
\end{table}

